A Miniature Batteryless Bioelectronic Implant Using One Magnetoelectric Transducer for Wireless Powering and PWM Backscatter Communication

Wireless minimally invasive bioelectronic implants enable a wide range of applications in healthcare, medicine, and scientific research. Magnetoelectric (ME) wireless power transfer (WPT) has emerged as a promising approach for powering miniature bio-implants because of its remarkable efficiency, safety limit, and misalignment tolerance. However, achieving low-power and high-quality uplink communication using ME remains a challenge. This paper presents a pulse-width modulated (PWM) ME backscatter uplink communication enabled by a switched-capacitor energy extraction (SCEE) technique. The SCEE rapidly extracts and dissipates the kinetic energy within the ME transducer during its ringdown period, enabling time-domain PWM in ME backscatter. Various circuit techniques are presented to realize SCEE with low power consumption. This paper also describes the high-order modeling of ME transducers to facilitate the design and analysis, which shows good matching with measurement. Our prototyping system includes a millimeter-scale ME implant with a fully integrated system-on-chip (SoC) and a portable transceiver for power transfer and bidirectional communication. SCEE is proven to induce >50% amplitude reduction within 2 ME cycles, leading to a PWM ME backscatter uplink with 17.73 kbps data rate and 0.9 pJ/bit efficiency. It also achieves 8.5 x 10 -5 bit-error-rate (BER) at a 5 cm distance, using a lightweight multi-layer-perception (MLP) decoding algorithm. Finally, the system demonstrates continuous wireless neural local-field potential (LFP) recording in an in vitro setup.

==> Comparison_table_new.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\begin{table*}[]
\caption{\textbf{Comparison with state-of-the-art mm-scale wireless implants with bidirectional telemetry.}}
\label{table}
\centering
\setlength{\tabcolsep}{3.6pt}
\renewcommand{\arraystretch}{1.5}
\begin{tabular}{|cc|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{2}{|c|}{\textbf{}} &
  \textbf{This work} &
  \begin{tabular}[c]{@{}c@{}}Z. Yu \\ MobiCom'22\cite{yu_magnetoelectric_2022}\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}J. Lim\\ VLSI'21\cite{lim_light-tolerant_2022}\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}J. Lee \\ Nat. Elec.'21\cite{lee_neural_2021}\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Y. Jia\\ ISSCC'20\cite{jia_trimodal_2020}\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}S. Sonmezoglu\\ ISSCC'20\cite{sonmezoglu_45mm3_2020}\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}M. Ghanbari\\ JSSC'19\cite{ghanbari_sub-mm3_2019}\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}S. Hosur\\ TBioCAS'23\cite{hosur_magsonic_2023}\end{tabular} \\ \hline
\multicolumn{2}{|c|}{\textbf{Biomedical Function}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Stimulation, \\ Recording\end{tabular}} &
  Stimulation &
  Recording &
  Recording &
  \begin{tabular}[c]{@{}c@{}}Stimulation, \\ Recording\end{tabular} &
  O\_2 sensing &
  Recording &
  N/A \\ \hline
\multicolumn{2}{|c|}{\textbf{SoC Technology (nm)}} &
  \textbf{180} &
  180 &
  180 &
  65 &
  350 &
  65 &
  65 &
  N/A \\ \hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{Power}}} &
  \textbf{Source} &
  \textbf{ME} &
  ME &
  Photodiode &
  RF &
  Inductive &
  Ultrasound &
  Ultrasound &
  MagSonic \\ \cline{2-10} 
\multicolumn{1}{|c|}{} &
  \textbf{Transfer Efficiency} &
  \textbf{0.37\% (2cm)} &
  0.2\% (2cm) &
  N/A &
  0.08\% (0.8cm) &
  N/A &
  N/A &
  0.06\% (1.8cm) &
  N/A \\ \hline
\multicolumn{1}{|c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Downlink \\ Data\end{tabular}}} &
  \textbf{Modality} &
  \textbf{ME} &
  ME &
  Photodiode &
  RF &
  Inductive &
  \multirow{2}{*}{N/A} &
  \multirow{2}{*}{N/A} &
  \multirow{2}{*}{N/A} \\ \cline{1-7}
\multicolumn{1}{|c|}{\textbf{}} &
  \textbf{Modulation} &
  \textbf{Time} &
  Time &
  PWM &
  PWM &
  OOK &
   &
   &
   \\ \hline
\multicolumn{1}{|c|}{\multirow{7}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Uplink \\ Data\end{tabular}}}} &
  \textbf{Modality} &
  \textbf{ME} &
  ME &
  LED &
  RF &
  RF &
  Ultrasound &
  Ultrasound &
  MagSonic \\ \cline{2-10} 
\multicolumn{1}{|c|}{} &
  \textbf{f\textsubscript{carrier} (kHz)} &
  \textbf{331} &
  335 &
  N/A &
  900000 &
  433000 &
  2000 &
  1780 &
  \begin{tabular}[c]{@{}c@{}}1930 \\ (Ultrasound)\end{tabular} \\ \cline{2-10} 
\multicolumn{1}{|c|}{} &
  \textbf{Modulation} &
  \textbf{\begin{tabular}[c]{@{}c@{}}PWM\\ Backscatter\end{tabular}} &
  \begin{tabular}[c]{@{}c@{}}LSK\\ Backscatter\end{tabular} &
  PGM &
  \begin{tabular}[c]{@{}c@{}}LSK\\ Backscatter\end{tabular} &
  OOK &
  \begin{tabular}[c]{@{}c@{}}LSK\\ Backscatter\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}AM\\ Backscatter\end{tabular} &
  OOK \\ \cline{2-10} 
\multicolumn{1}{|c|}{} &
  \textbf{Data Rate (kbps)} &
  \textbf{17.73} &
  1.6 &
  0.3 &
  10000 &
  6780 &
  60 &
  35 &
  100 \\ \cline{2-10} 
\multicolumn{1}{|c|}{} &
  \textbf{Data Rate / f\textsubscript{carrier}} &
  \textbf{0.054} &
  0.0047 &
  N/A &
  0.011 &
  0.0156 &
  0.03 &
  0.0197 &
  0.0518 \\ \cline{2-10} 
\multicolumn{1}{|c|}{} &
  \textbf{Bit Energy (pJ/Bit)} &
  \textbf{0.9} &
  N/A &
  253 &
  N/A &
  1342.2 &
  55 &
  603 &
  190 \\ \cline{2-10} 
\multicolumn{1}{|c|}{} &
  \textbf{BER} &
  \textbf{8.5E-5 (5cm)} &
  9E-4 (1.5cm) &
  N/A &
  5E-3 (0.8cm) &
  N/A &
  9E-5 (5cm) &
  N/A &
  1E-5 (4cm) \\ \hline
\multicolumn{2}{|c|}{\textbf{Max Distance (cm)}} &
  \textbf{5} &
  2 &
  N/A &
  0.8 &
  N/A &
  5 &
  5 &
  4 \\ \hline
\end{tabular}
\end{table*}

==> Modeling.tex <==
\section{Modeling of ME Transducer} \label{modeling_section}

\subsection{Basic ME Model}

The design of the energy extraction interface for the PWM backscatter requires an electrical model of the ME transducer to study the effect of the modulation on the transducer's behavior. 

Similar to the ultrasonic transducer, which converts acoustic waves to electrical fields, we can employ \textit{Van Dyke} circuit to model the electro-acoustic impedance~\cite{noauthor_ieee_1978}. Additionally, a transformer is included to represent the conversion from magnetic waves to acoustic waves, as shown in Fig.~\ref{Original_model}. To obtain the parameters for this model, we first measure the output impedance of the ME film using a Vector Network Analyzer (VNA). With the ME film not being actively driven, the source is set to zero, simplifying the model to that shown in Fig.~\ref{Input_impedance}. The collected data is then fit into the impedance model. Fig.~\ref{1st_order_fitting} shows an example of the fitting curves of the ME film we used in this design, along with the obtained model parameters. This model is subsequently utilized in circuit simulations to determine design parameters, such as the value of the flying capacitors in the SCEE interface.

\begin{figure}[t!]
%\vskip -3ex
\centering
\subfloat[]{\includegraphics[scale = 0.4]{Figure_added/Original_model.pdf}%
\label{Original_model}}\\
\subfloat[]{\includegraphics[scale = 0.4]{Figure_added/Original_impedance.pdf}%
\label{Input_impedance}}\\
\caption{(a) Circuit model of ME transducer; (b) Simplified impedance model of ME transducer.}
\label{Models}
\end{figure}


\begin{figure}[t!]
%\vskip -3ex
\centering
\includegraphics[scale = 0.25]{Figure_added/1st_order_impedance_fitting.pdf}
\vskip -2ex
\caption{Impedance fitting of an ME film and the corresponding model parameters, where $f_{sc}$ and $f_{oc}$ are the short-circuit and open-circuit resonance frequency calculated from the impedance model parameters.}
\label{1st_order_fitting}
\end{figure}

With the model in Fig.~\ref{Input_impedance}, we simulated the SCEE interface circuit. The energy extraction is performed 8 times when the external field is turned off. For simplicity, No rectifier is connected, so there is no voltage clamping. Fig.~\ref{VAC_1st} shows the simulation waveform of the ME transducer voltage. As can be seen, the $V_{AC}$ waveform with the basic model is regular after voltage flipping. The voltage flipping point is aligned well with the peak, and the amplitude is significantly reduced. 



\begin{figure}[t!]
%\vskip -3ex
\centering
\includegraphics[scale = 0.24]{Figure_added/VAC_1st.pdf}
\vskip -2ex
\caption{Simulated ME transducer voltage with the SCEE interface using the basic circuit model.}
\label{VAC_1st}
\end{figure}





\begin{figure}[t!]
%\vskip -3ex
\centering
\includegraphics[scale = 0.24]{Figure_added/VAC_meas.pdf}
\vskip -2ex
\caption{Measured $V_{AC}$ waveform with SCEE.}
\label{VAC_meas}
\end{figure}



\begin{figure}[t!]
%\vskip -3ex
\centering
\includegraphics[scale = 0.4]{Figure_added/high_order_impedance.pdf}
\vskip -2ex
\caption{High-order ME impedance model that consists of N vibration modes.}
\label{high_order_impedance}
\end{figure}


\begin{figure}[t!]
%\vskip -3ex
\centering
\includegraphics[scale = 0.23]{Figure_added/3rd_order_impedance_fitting.pdf}
\vskip -2ex
\caption{Impedance measurement and fitting up to 2 MHz and the corresponding parameters of the 3rd order impedance model.}
\label{3rd_order_fitting}
\end{figure}

\begin{figure}[t!]
%\vskip -3ex
\centering
\includegraphics[scale = 0.24]{Figure_added/VAC_3rd.pdf}
\vskip -2ex
\caption{Simulated $V_{AC}$ waveform with SCEE.}
\label{VAC_3rd}
\end{figure}

\subsection{High-Order ME Model}

Before designing the SoC, a printed circuit board (PCB)-level SCEE prototype is made and tested. The PCB contains MOSFET switches, flying capacitors, and switch drivers. However, the testing result deviates from the simulation result obtained using the basic model. Fig.~\ref{VAC_meas} shows the measured $V_{AC}$ waveform, scaled to have a similar amplitude as in Fig.~\ref{VAC_1st}. After voltage flipping, the transducer voltage amplitude first decreases and then increases in the opposite direction. Moreover, frequency components that are higher than the carrier appear after voltage flipping. Despite completing the SCEE process, high-frequency signals persist for several cycles. The peak points become difficult to distinguish, and the residual voltage after SCEE is higher than that of the basic model. These phenomena motivated us to build a more accurate model to investigate the energy extraction process of the ME transducers.
Based on the observation from the measurement that the waveform contains high-frequency components, we intended to use a higher-order model to emulate the ME transducer's behavior. Prior works have demonstrated the second vibration mode of the ME transducer and utilized it in the active driving uplink communication method \cite{hosur_magsonic_2023}. However, there is no circuit model in the literature that describes the other vibration modes. Here, we present a new ME model that well emulates the effect of high-frequency vibration modes in energy extraction and can potentially extend to other designs. 

The primary vibration mode of an ME film is the length mode, which operates at a low frequency of hundreds of kilohertz. However, the ME film also exhibits piezoelectric effects in other directions, such as width and thickness. These modes have higher frequencies and generally contribute minimally to the ME transducer voltage when driven by a magnetic field, as they are far off-resonance. During energy extraction, however, the interface circuit induces sudden drops in ME voltage. This not only extracts energy from the main resonance mode but also excites other resonance modes due to the wide bandwidth of the pulse-like waveform. Consequently, these additional resonance modes significantly influence the energy extraction process.

To model the effects of high-frequency resonance modes, the high-order ME impedance model is proposed, as shown in Fig.~\ref{high_order_impedance}. In this model, each resonance is represented by an impedance $Z_{m}$, where the $R_m$, $L_m$, and $C_m$ correspond to damping, mass, and stiffness in the mechanical domain. $C_p$ is the lumped electrical parasitic capacitor between the two ME terminals. 
Using this model, we can analyze the ME transducer's behavior in SCEE through simulation tools. Note that this model does not include input sources in each branch, as the external TX is turned off during SCEE. However, if we need to examine the behavior when the ME film is powered by a magnetic wave, we can reintroduce the sinusoidal source and transformer to the main resonance branch while treating the other branches as loads.

The impedance measurement up to 2 MHz of the same ME film as in Fig.~\ref{1st_order_fitting} and the model fitting results are depicted in Fig.~\ref{3rd_order_fitting}. The impedance curves show three dominant resonance peaks. Therefore, a 3rd-order impedance model was selected for fitting. The fitting results align well with the impedance measurement across both low and high frequencies.



The 3rd-order model is simulated with the SECC interface circuit to verify the proposed model, as shown in Fig.~\ref{VAC_3rd}. Although the voltage waveform is not exactly the same because of slightly different setups, we can notice several features that match the waveform in Fig.~\ref{VAC_meas}. Firstly, the $V_{AC}$ voltage shows a reversion right after each voltage flipping. Secondly, when the whole SCEE process is done, the $V_{AC}$ waveform is still distorted for a few cycles, which is more severe in the simulation. These features are induced by the higher-frequency resonance excited by the SCEE operation, which has justified the proposed high-order ME model. 



Despite the non-ideal behavior caused by the high-frequency resonance, the SCEE still effectively reduces the voltage amplitude in the ME transducer. According to the simulation results in Fig.~\ref{VAC_1st} and Fig.~\ref{VAC_3rd}, the amplitude reduction effect decreases by 8.9\% (from 82.4\% to 73.5\%) when using the high-order model. This slight decline does not impact the operation of the PWM backscatter. Additionally, as demonstrated in the measurement results in Section \ref{measurement}, the backscattered signal maintains good quality, and the prototype achieves high accuracy over long distances.








==> Modeling_bk.tex <==
\section{Modeling of ME Transducer} \label{modeling_section}

\subsection{Basic ME Model}

The design of the energy extraction interface for the PWM backscatter requires an electrical model of the ME transducer to study the effect of such modulation on the transducer's behavior. Similar to the ultrasonic transducer, which converts acoustic waves to electrical fields, we can employ \textit{Van Dyke} circuit to model the electro-acoustic impedance. Additionally, a transformer is included to represent the conversion from magnetic waves to acoustic waves, as shown in Fig.~\ref{Original_model}. To obtain the parameters for this model, we first measure the output impedance of the ME film using a Vector Network Analyzer (VNA). With the ME film not being actively driven, the source is set to zero, simplifying the model to that shown in Fig.~\ref{Input_impedance}. The collected data is then fit into the impedance model. Fig.~\ref{1st_order_fitting} shows an example of the fitting curves of the ME film we used in this design, along with the obtained model parameters. This model is subsequently utilized in circuit simulations to determine design parameters, such as the value of the flying capacitors in the SCEE interface.

\begin{figure}[t!]
%\vskip -3ex
\centering
\subfloat[]{\includegraphics[scale = 0.4]{Figure_added/Original_model.pdf}%
\label{Original_model}}\\
\subfloat[]{\includegraphics[scale = 0.4]{Figure_added/Original_impedance.pdf}%
\label{Input_impedance}}\\
\caption{(a) Circuit model of ME transducer; (b) Simplified impedance model of ME transducer.}
\label{Models}
\end{figure}


\begin{figure}[t!]
%\vskip -3ex
\centering
\includegraphics[scale = 0.25]{Figure_added/1st_order_impedance_fitting.pdf}
\vskip -2ex
\caption{Impedance fitting of an ME film and the corresponding model parameters, where $f_{sc}$ and $f_{oc}$ are the short-circuit and open-circuit resonance frequency calculated from the impedance model parameters.}
\label{1st_order_fitting}
\end{figure}

However, during testing, we found that the measured waveform of ME transducer voltage during the energy extraction deviates from the results simulated with the impedance model in Fig.~\ref{Input_impedance}. After voltage flipping, the transducer voltage would first decrease and then increase toward the other direction. When the flipping process is ongoing or is just finished, the transducer voltage is not strictly sinusoidal but distorted. This phenomenon motivated us to build a more accurate model to investigate the energy extraction of the ME transducer. Based on the observation from the measurement that the waveform contains other frequency components, we intended to use a higher-order model to emulate the ME transducer's behavior. Actually, prior works have demonstrated the second vibration mode of the ME transducer and utilized it in the active driving communication method \cite{hosur_magsonic_2023}. However, there is no circuit model in the literature that describes the other vibration modes. Here, we present a new ME model that well emulates the effect of high-frequency vibration modes in energy extraction and can potentially extend to other designs.


\subsection{High-Order ME Model}


The primary vibration mode of an ME film is the length mode, which operates at a low frequency of hundreds of kilohertz. However, the film also exhibits piezoelectric effects in other directions, such as width and thickness. These modes have higher frequencies and generally contribute minimally to the ME transducer voltage when driven by a magnetic field, as they are far off-resonance. During energy extraction, however, the interface circuit induces sudden drops in ME voltage. This not only extracts energy from the main resonance mode but also excites other resonance modes due to the wide bandwidth of the pulse-like waveform. Consequently, these additional resonance modes significantly influence the energy extraction process.

To model the effects of high-frequency resonance modes, the high-order ME impedance model is proposed, as shown in Fig.~\ref{high_order_impedance}. In this model, each resonance is represented by an impedance $Z_{m}$, where the $R_m$, $L_m$, and $C_m$ correspond to damping, mass, and stiffness in the mechanical domain. $C_p$ is the lumped electrical parasitic capacitor between the two ME terminals. 
%During each energy extraction phase, when the voltage across $C_p$ is flipped, the high-frequency modes are excited, and current will flow in each branch. 
%Using this model, we can study the ME transducer's behavior in SCEE using simulation tools. Noted that this model does not contain the input sources in each branch. This is because during SCEE, the external TX is turned off. But if we need to study the behavior when the ME film is powered by the magnetic wave, we can add the sinusoidal source and the transformer back to the main resonance branch and other branches are treated as load.
Using this model, we can analyze the ME transducer's behavior in SCEE through simulation tools. Noted that this model does not include input sources in each branch, as the external TX is turned off during SCEE. However, if we need to examine the behavior when the ME film is powered by a magnetic wave, we can reintroduce the sinusoidal source and transformer to the main resonance branch while treating the other branches as loads.

The impedance measurement up to 2 MHz of the same ME film as in Fig.~\ref{1st_order_fitting} and the model fitting results are depicted in Fig.~\ref{3rd_order_fitting}. The impedance curves show three dominant resonance peaks. Therefore, a 3rd-order impedance model was selected for fitting. The fitting results align well with the impedance measurement across both low and high frequencies.


\begin{figure}[t!]
%\vskip -3ex
\centering
\includegraphics[scale = 0.42]{Figure_added/high_order_impedance.pdf}
\vskip -2ex
\caption{High-order ME impedance model that consists of N vibration modes.}
\label{high_order_impedance}
\end{figure}


\begin{figure}[t!]
%\vskip -3ex
\centering
\includegraphics[scale = 0.23]{Figure_added/3rd_order_impedance_fitting.pdf}
\vskip -2ex
\caption{Impedance measurement and fitting up to 2 MHz and the corresponding parameters of the 3rd order impedance model.}
\label{3rd_order_fitting}
\end{figure}




\subsection{Simulation Results}


The basic ME model and the 3rd-order model are simulated with the SECC interface circuit to verify the proposed model, as shown in Fig.~\ref{VACs}. The external magnetic field is turned off at 30 $\mu s$ and SCEE is triggered at around 31 $\mu s$ in both cases. No rectifier is connected in the setup, so there is no voltage clamping, for simplicity. As can be seen, the $V_{AC}$ waveform with the basic model is regular after voltage flipping. The voltage flipping point is aligned well with the peak, and the amplitude is significantly reduced. On the other hand, with the 3rd-order model, frequency components that are higher than the carrier appear after voltage flipping. Even if the SCEE is done (8 voltage flipping in total), the high-frequency signals remain for several cycles. The peak points become difficult to distinguish, and the residual voltage after SCEE is higher than the basic model case. 

\begin{figure}[t!]
%\vskip -3ex
\centering
\subfloat[]{\includegraphics[scale = 0.25]{Figure_added/VAC_1st.pdf}%
\label{VAC_1st}}\\
\subfloat[]{\includegraphics[scale = 0.25]{Figure_added/VAC_3rd.pdf}%
\label{VAC_3rd}}\\
\caption{Simulated $V_{AC}$ waveforms with SCEE using (a) basic model and (b) 3rd-order model.}
\label{VACs}
\end{figure}



\begin{figure}[t!]
%\vskip -3ex
\centering
\includegraphics[scale = 0.255]{Figure_added/VAC_meas.pdf}
\vskip -2ex
\caption{Measured $V_{AC}$ waveform with SCEE.}
\label{VAC_meas}
\end{figure}


\begin{figure*}[t!]
%\vskip -3ex
\centering
\includegraphics[scale = 0.83]{Figure/System_diagram.pdf}
\vskip -1ex
\caption{System diagram of the ME implant SoC and the PWM ME backscatter module.}
\label{system_diagram}
\end{figure*}

Fig.~\ref{VAC_meas} shows the measured $V_{AC}$ waveform with the SCEE interface circuit. Although the voltage waveform is not exactly the same because of different setups, we can notice several features that match the waveform in Fig.~\ref{VAC_3rd}. Firstly, the $V_{AC}$ voltage shows a reversion right after each voltage flipping. Secondly, when the whole SCEE process is done, the $V_{AC}$ waveform is still distorted for a few cycles, which is more severe in the simulation. These features are induced by the higher-frequency resonance excited by the SCEE operation, which has justified the proposed high-order ME model. Although the high-order resonance modes cause some non-idealities for the energy extraction, the backscattered signal still has good quality according to the experimental results shown in Section \ref{measurement}.



==> table_figure.tex <==
\begin{table*}[t]
\begin{center}
\caption{\textbf{Comparisons with State-of-the-Art WPT Technologies for Biomedical Implants}}
\includegraphics[width=7in]{Figure/table.png}
\label{tab1}
\end{center}
\end{table*}
